Quantum Semantic Correlations in Hate and Non-Hate Speeches

This paper aims to apply the notions of quantum geometry and correlation to the typification of semantic relations between couples of keywords in different documents. In particular we analysed texts classified as hate / non hate speeches, containing the keywords "women", "white", and "black". The paper compares this approach to cosine similarity, a classical methodology, to cast light on the notion of "similar meaning".

==> eptcsdata.tex <==
\providecommand{\firstpage}{62}
\providecommand{\publicationstatus}{B. Coecke, J. Hedges, D. Kartsaklis, M. Lewis, D. Marsden (Eds.):\\2018 Workshop on Compositional Approaches\\for Physics, NLP, and Social Sciences (CAPNS)\\
EPTCS 283, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.283.5}{10.4204/EPTCS.283.5}}
\pdfoutput=1

